"A good pun is its own reword": Can Large Language Models Understand Puns?

Puns play a vital role in academic research due to their distinct structure and clear definition, which aid in the comprehensive analysis of linguistic humor. However, the understanding of puns in large language models (LLMs) has not been thoroughly examined, limiting their use in creative writing and humor creation. In this paper, we leverage three popular tasks, i.e., pun recognition, explanation and generation to systematically evaluate the capabilities of LLMs in pun understanding. In addition to adopting the automated evaluation metrics from prior research, we introduce new evaluation methods and metrics that are better suited to the in-context learning paradigm of LLMs. These new metrics offer a more rigorous assessment of an LLM's ability to understand puns and align more closely with human cognition than previous metrics. Our findings reveal the "lazy pun generation" pattern and identify the primary challenges LLMs encounter in understanding puns.

==> 100response.tex <==
We thank all reviewers for your valuable guidance in improving our paper. We have carefully considered all the suggestions, and have made the following revisions to the paper:


\section{Response to Reviewer fnPc}
Based on your constructive feedback, we have made the following revisions to our paper:
\begin{enumerate}
    \item Add the shortcomings of the Overlap metric in the Limitations section. It is a rough indicator of originality and not an exact measurement.
    \item Provide more information about our annotators in Appendix A.
    \item Adjust the x-axe labels of Figures 4 and 5 for better clarity.
\end{enumerate}


\section{Response to Reviewer KVZ6}
According to your helpful comments, we have made the following revisions to our paper:
\begin{enumerate}
    \item Add the comparison of hom-pun and het-pun results across different tasks.
    \item Reduce the use of GPT-4 as an evaluator (see Section 4.5.3 Metrics for Generation) to minimize the potential bias.
    \item Adjust the legend in Figure 5 to make it no longer cover the graph.
\end{enumerate}


\section{Response to Reviewer W4Yo}
We appreciate your detailed suggestions and have made the following revisions accordingly:

\paragraph{Major Revisions}
\begin{enumerate}
    \item Add human evaluation for the generation task. We ask our annotators to label the success (0/1) and funniness (1-5) of human puns and llm-generated puns (see Section 4.5.3).
    \item Acknowledge the limitation of the Overlap metric as it is not a precise measurement for LLM's originality (see Limitations section).
    \item Add more information about our annotators' backgrounds in Appendix A.
    \item State it clear in Sections 4.1 and 4.2 that free generation and constrained generation refer to the use of context words.
\end{enumerate}

\paragraph{Minor Revisions}
\begin{enumerate}
    \item Remove the discussion in Section 5.1 regarding ``OpenChat-7B outperforms Gemini-Pro and GPT-3.5-Turbo''.
    \item Remove the content about ``human cognition'' to avoid confusion.
    \item Adjust the bold and underline in Table 2 for $\Delta_{TPR}$ and $\Delta_{TNR}$ to show our preference for smaller variations.
    \item Adjust the legend and x-axe labels of Figure 5 for better clarity.
    \item Polish other less precise or bold statements. Fix typos.  
\end{enumerate}



==> tables/042correlation.tex <==
\setlength\tabcolsep{1.5pt}
\begin{table}[t]
  \centering
  \small
    \begin{tabular}{lccc}
    \toprule
    \textbf{Evaluation Task} & Pearson's $r$ & Spearman's $\rho$ & Kendall's $\tau$ \\
    \midrule
    Pairwise Comparison & 0.687 & 0.718 & 0.707 \\
    Generation Success  & 0.816 & 0.816 & 0.816 \\
    \bottomrule
    \end{tabular}
    \caption{Correlation metrics between human and GPT-4 assessment in different evaluation tasks.}
  \label{tab:correlation}
\end{table}



==> tables/053pairwisecomparison.tex <==
\setlength\tabcolsep{1.8pt}
\begin{table}[t]
  \centering
  \small
    \begin{tabular}{lmmmttt}
    \toprule
    \textbf{Human vs} & \multicolumn{3}{c}{\textbf{Homographic Pun}} & \multicolumn{3}{c}{\textbf{Heterographic Pun}} \\
    \cmidrule(lr){2-4}  \cmidrule(lr){5-7}
    \rowcolor{white} \textbf{Model}  & Tie & Human & Model & Tie & Human & Model \\
    \midrule
    Llama2-7B-Chat & 0.307 & \textbf{0.585} & 0.107 & 0.096 & \textbf{0.841} & 0.063 \\
    Vicuna-7B & 0.351 & \underline{0.568} & 0.082 & 0.170  & \underline{0.779} & 0.051 \\
    Mistral-7B & 0.380  & 0.523 & 0.096 & 0.187 & 0.759 & 0.054 \\
    OpenChat-7B & 0.505 & 0.338 & 0.157 & 0.240  & 0.689 & 0.071 \\
    \cdashlinelr{1-7}
    Gemini-Pro & 0.653 & 0.165 & 0.181 & 0.417 & 0.461 & 0.122 \\
    GPT-3.5-Turbo & 0.668 & 0.172 & 0.161 & 0.445 & 0.442 & 0.113 \\
    GPT-4-Turbo & \textbf{0.769} & 0.017 & \underline{0.214} & \textbf{0.685} & 0.087 & \underline{0.229} \\
    Claude-3-Opus & \underline{0.733} & 0.041 & \textbf{0.226} & \underline{0.644} & 0.121 & \textbf{0.235} \\
    \bottomrule
    \end{tabular}%
    \caption{Results of pairwise comparison for pun explanations.}
    \label{tab:pairwisecomparison}
\end{table}%


